Many Roads Lead to Lithium: Formation Pathways For Lithium-Rich Red Giants

Stellar models predict that lithium (Li) inside a star is destroyed during the first dredge-up phase, yet 1.2% of red giant stars are Li-rich. We aim to uncover possible origins of this population, by analysing 1155 Li-rich giants (A(Li) $\geq$ 1.5) in GALAH DR3. To expose peculiar traits of Li-rich stars, we construct a reference sample of Li-normal (doppelg\"anger) stars with matched evolutionary state and fiducial supernova abundances. Comparing Li-rich and doppelg\"anger spectra reveals systematic differences in the H-$\alpha$ and Ca-triplet line profiles associated with the velocity broadening measurement. We also find twice as many Li-rich stars appear to be fast rotators (2% with $v_\textrm{broad} \gtrsim 20$ km s$^{-1}$) compared to doppelg\"angers. On average, Li-rich stars have higher abundances than their doppelg\"angers, for a subset of elements, and Li-rich stars at the base of RGB have higher mean $s-$process abundances ($\geq 0.05$ dex for Ba, Y, Zr), relative to their doppelg\"angers. External mass-transfer from intermediate-mass AGB companions could explain this signature. Additional companion analysis excludes binaries with mass ratios $\gtrsim$ 0.5 at $\gtrsim$ 7 AU. We also discover that highly Ba-enriched stars are missing from the Li-rich population, possibly due to low-mass AGB companions which preclude Li-enrichment. Finally, we confirm a prevalence of Li-rich stars on the red clump that increases with lithium, which supports an evolutionary state mechanism for Li-enhancement. Multiple culprits, including binary spin-up and mass-transfer, are therefore likely mechanisms of Li-enrichment.

==> format.tex <==

\begin{itemize}
    \setlength\itemsep{0em}
    \setlength\parskip{0em}
    \item \textbf{Start with stellar evolution}
    \begin{itemize}
        \setlength\itemsep{0em}
        \setlength\parskip{0em}
        \item how does a star evolve from MS to RG phase; incl. dredge-up, helium flash
        \item what happens to elements from MS to RG phase; incl. elements produced/destroyed b/c of temp \& mixing
    \end{itemize}
    \item \textbf{Mention the lithium-enrichment problem}
    \begin{itemize}
        \setlength\itemsep{0em}
        \setlength\parskip{0em}
        \item ways to increase \ali
        \item explain cameron-fowler 
        \item planet engulfment, spin-up, more 
    \end{itemize}
    \item \textbf{what has been done in the past?}
    \begin{itemize}
        \setlength\itemsep{0em}
        \setlength\parskip{0em}
        \item \citep{martell_2021}
        \item see papers below
    \end{itemize}
    \item \textbf{what do we do differently? why was it needed?}
    \begin{itemize}
        \setlength\itemsep{0em}
        \setlength\parskip{0em}
        \item we have TESS so more stars
        \item \dg sample
    \end{itemize}
\end{itemize}

